Fine-Grained Analysis of Optimization and Generalization for Overparameterized Two-Layer Neural Networks

Recent works have cast some light on the mystery of why deep nets fit any data and generalize despite being very overparametrized. This paper analyzes training and generalization for a simple 2-layer ReLU net with random initialization, and provides the following improvements over recent works: (i) Using a tighter characterization of training speed than recent papers, an explanation for why training a neural net with random labels leads to slower training, as originally observed in [Zhang et al. ICLR'17]. (ii) Generalization bound independent of network size, using a data-dependent complexity measure. Our measure distinguishes clearly between random labels and true labels on MNIST and CIFAR, as shown by experiments. Moreover, recent papers require sample complexity to increase (slowly) with the size, while our sample complexity is completely independent of the network size. (iii) Learnability of a broad class of smooth functions by 2-layer ReLU nets trained via gradient descent. The key idea is to track dynamics of training and generalization via properties of a related kernel.

==> opt_perturbation.tex <==
We first consider the continuous time gradient flow.
The key idea is to consider the following auxiliary ODEs\begin{align*}
\frac{d\widetilde{\mat{W}}(t)}{dt} = &- \mat{Z}(0) \left(\tilde{\vect{u}}(t)-\vect{y}\right) \text{ with } \widetilde{\mat{W}} = \mat{W}(0) \\
\frac{d\tilde{\vect{u}}(t)}{dt} = &- \mat{H}(0)\left(\tilde{\vect{u}}(t)-\vect{y}\right) \text{ and }\tilde{\vect{u}}(0) = \vect{u}(0).
\end{align*} 

Note $\widetilde{\mat{W}}(t)$ is the desired ODE, so we want to bound $\mat{W}-\widetilde{\mat{W}}(t)$.
\begin{lem}\label{lem:gf_optimization}
With high probability over initialization, we have for all $t\ge 0$\begin{align*}
	\norm{\mat{W}(t)-\widetilde{\mat{W}}(t)}_F \le \frac{\poly(n,1/\lambda_0,\log m)}{\sqrt{m}}.
\end{align*}
\end{lem}



Also note, both $\vect{u}(t)-\tilde{\vect{u}}(t)$ will converge to $\vect{y}$ by the analysis in \cite{du2018provably}.
We can compute \begin{align*}
&\frac{d \left(\mat{W}(t)-\widetilde{\mat{W}}(t)\right)}{dt}\\
= &-\mat{Z}(t)(\vect{u}(t)-\vect{y}) + \mat{Z}(0)\left(\tilde{\vect{u}}(t)-\vect{y}\right) \\
= &\left(\mat{Z}(0)-\mat{Z}(t)\right)\left(\vect{u}(t)-\vect{y}\right) + \mat{Z}(0)\left(\tilde{\vect{u}}(t)-\vect{u}(t)\right).
\end{align*}
For the first term, recall in \cite{du2018provably}, they showed for all $t >0$ \begin{align*}
	\norm{\mat{Z}(t) - \mat{Z}(0)}_2 = \frac{\poly(n,1/\lambda_0)}{\sqrt{m}}.
\end{align*}
Therefore we can bound \begin{align*}
	\int \norm{\left(\mat{Z}(0)-\mat{Z}(t)\right)\left(\vect{u}(t)-\vect{y}\right) }_F dt \le \frac{\poly(n,1/\lambda_0)}{\sqrt{m}} \int \norm{\tilde{\vect{u}}(t)-\vect{y}}_2 dt= \frac{\poly(n,1/\lambda_0)}{\sqrt{m}}.
\end{align*}
For the second term, we thus need to bound\begin{align}
\int_{t=0}^{\infty}\norm{\tilde{\vect{u}}(t)-\vect{u}(t)}_2 dt. \label{eqn:u_tilde_u}
\end{align}
To bound Equation~\eqref{eqn:u_tilde_u}, we observe that $\tilde{\vect{u}}(t) \rightarrow \vect{y}$ and $\vect{u}(t) \rightarrow \vect{y}$.
Therefore, we can choose some $t_0$ such that \begin{align*}
\int_{t_0}^\infty\norm{\vect{\tilde{u}}(t)-\vect{u}(t)}_2 dt \le \int_{t_0}^\infty(\norm{\vect{\tilde{u}}(t)-\vect{y}}_2  + \norm{\vect{y}-\vect{u}(t)}_2 )dt
\end{align*}
Note if we choose $t_0 = \frac{C}{\lambda_0}\left(\frac{m\lambda_0}{n}\right)$ so that \begin{align*}
\int_{t_0}^\infty\norm{\vect{\tilde{u}}(t)-\vect{u}(t)}_2 dt \le \frac{2\norm{\vect{u}(t)-\vect{y}}_2}{\lambda_0} \le \frac{\poly(n,1/\lambda_0)}{\sqrt{m}}.
\end{align*}
Thus it suffices to bound \begin{align*}
	\int_{t=0}^{t_0}\norm{\tilde{\vect{u}}(t)-\vect{u}(t)}_2 dt \le t_0 \max_{0\le t\le t_0} \norm{\tilde{\vect{u}}(t)-\vect{u}(t)}_2.
\end{align*}
First observe that \[
 \norm{\tilde{\vect{u}}(t)-\vect{u}(t)}_2 \le \int_{\tau = 0}^t \norm{\frac{d\left(\tilde{\vect{u}}(\tau)-\vect{u}(\tau)\right)}{d \tau}}_2 d\tau.
 \]
 Note \begin{align*}
 &\frac{d \left(\tilde{\vect{u}}(t)-\vect{u}(t)\right)}{dt} \\
 = &-\mat{H}(0)\left(\tilde{\vect{u}}(t)-\vect{y}\right) + \mat{H}(t)\left(\vect{u}(t)-\vect{y}\right) \\
 = &  -\mat{H}(0)\left(\tilde{\vect{u}}(t)-\vect{u}(t)\right) + \left(\vect{u}(t)-\vect{y}\right)\left(\mat{H}(t)-\mat{H}(0)\right).
 \end{align*}
Since $\mat{H}(0)$ is positive semidefinite, $-\mat{H}(0)\left(\tilde{\vect{u}}(t)-\vect{u}(t)\right) $ term only makes $\norm{\tilde{\vect{u}}(t)-\vect{u}(t)}_2$ smaller.
Therefore, we have \begin{align*}
\norm{\tilde{\vect{u}}(t)-\vect{u}(t)}_2 \le &\int_{\tau =0}^t \norm{\vect{u}(\tau)-\vect{y}}_2 \norm{\mat{H}(t)-\mat{H}(0)}_2 \\
\le & t\norm{\vect{u}(0)-\vect{y}}_2 \frac{\poly(n,1/\lambda_0)}{\sqrt{m}} = \frac{t\poly(n,1/\lambda_0)}{\sqrt{m}} .
\end{align*}
Therefore, we have \begin{align*}
	\int_{t=0}^{t_0}\norm{\tilde{\vect{u}}(t)-\vect{u}(t)}_2 dt \le t_0 \max_{0\le t\le t_0} \norm{\tilde{\vect{u}}(t)-\vect{u}(t)}_2 \le t_0^2 \frac{\poly(n,1/\lambda_0)}{\sqrt{m}} \le \frac{\poly(n,1/\lambda_0,\log(m))}{\sqrt{m}}.
\end{align*}
\qed

==> proof_sketch.tex <==
\begin{proof}[Proof Sketch of Theorem~\ref{thm:traj_u}]
Here we give a continuous time proof of Theorem~\ref{thm:traj_u}.
The discrete time proof follows similar ideas but involves more (non-trivial) perturbation analysis so we deferred it to appendix. 

Note for continuous time we have the following differential equations\begin{align*}
\frac{d \vect{u}(t)}{dt} = &-\mat{H}(t)\left(\vect{u}(t)-\vect{y}\right), \\
\frac{d \tilde{\vect{u}}(t)}{dt} = &- \mat{H}^{\infty}\left(\tilde{\vect{u}}(t)-\vect{y}\right).
\end{align*}

First observe that because $\tilde{\vect{u}}(0) = \vect{u}(0)$, we have \[
\norm{\tilde{\vect{u}}(t)-\vect{u}(t)}_2 \le \int_{\tau = 0}^t \norm{\frac{d\left(\tilde{\vect{u}}(\tau)-\vect{u}(\tau)\right)}{d \tau}}_2 d\tau.
\]
Note \begin{align*}
&\frac{d \left(\tilde{\vect{u}}(t)-\vect{u}(t)\right)}{dt} \\
= &-\mat{H}(0)\left(\tilde{\vect{u}}(t)-\vect{y}\right) + \mat{H}(t)\left(\vect{u}(t)-\vect{y}\right) \\
= &  -\mat{H}(0)\left(\tilde{\vect{u}}(t)-\vect{u}(t)\right) + \left(\vect{u}(t)-\vect{y}\right)\left(\mat{H}(t)-\mat{H}(0)\right).
\end{align*}
Since $\mat{H}(0)$ is positive semidefinite, $-\mat{H}(0)\left(\tilde{\vect{u}}(t)-\vect{u}(t)\right) $ term only makes $\norm{\tilde{\vect{u}}(t)-\vect{u}(t)}_2$ smaller.
Therefore, we have \begin{align*}
&\norm{\tilde{\vect{u}}(t)-\vect{u}(t)}_2 \\
\le &\int_{\tau =0}^t \norm{\vect{u}(\tau)-\vect{y}}_2 \norm{\mat{H}(t)-\mat{H}(0)}_2 \\
\le & t\norm{\vect{u}(0)-\vect{y}}_2 \frac{\poly(n,1/\lambda_0)}{\sqrt{m}} = \frac{t\poly(n,1/\lambda_0)}{\sqrt{m}} .
\end{align*}

\end{proof}




\begin{proof}[Proof Sketch of Theorem~\ref{thm:traj_W}]
	To illustrate the main proof idea we give the continuous time analysis below.
	We first consider the continuous time gradient flow.
	The key idea is to consider the following auxiliary ODEs\begin{align*}
	\frac{d\widetilde{\mat{W}}(t)}{dt} = &- \mat{Z}(0) \left(\tilde{\vect{u}}(t)-\vect{y}\right) \text{ with } \widetilde{\mat{W}} = \mat{W}(0) \\
	\frac{d\tilde{\vect{u}}(t)}{dt} = &- \mat{H}(0)\left(\tilde{\vect{u}}(t)-\vect{y}\right) \text{ and }\tilde{\vect{u}}(0) = \vect{u}(0).
	\end{align*} 
	
	Note $\widetilde{\mat{W}}(t)$ is the desired ODE, so we want to bound $\mat{W}-\widetilde{\mat{W}}(t)$.
	\begin{lem}\label{lem:gf_optimization}
		With high probability over initialization, we have for all $t\ge 0$\begin{align*}
		\norm{\mat{W}(t)-\widetilde{\mat{W}}(t)}_F \le \frac{\poly(n,1/\lambda_0,\log m)}{\sqrt{m}}.
		\end{align*}
	\end{lem}
	
	
	
	Also note, both $\vect{u}(t)-\tilde{\vect{u}}(t)$ will converge to $\vect{y}$ by the analysis in \cite{du2018provably}.
	We can compute \begin{align*}
	&\frac{d \left(\mat{W}(t)-\widetilde{\mat{W}}(t)\right)}{dt}\\
	= &-\mat{Z}(t)(\vect{u}(t)-\vect{y}) + \mat{Z}(0)\left(\tilde{\vect{u}}(t)-\vect{y}\right) \\
	= &\left(\mat{Z}(0)-\mat{Z}(t)\right)\left(\vect{u}(t)-\vect{y}\right) + \mat{Z}(0)\left(\tilde{\vect{u}}(t)-\vect{u}(t)\right).
	\end{align*}
	For the first term, recall in \cite{du2018provably}, they showed for all $t >0$ \begin{align*}
	\norm{\mat{Z}(t) - \mat{Z}(0)}_2 = \frac{\poly(n,1/\lambda_0)}{\sqrt{m}}.
	\end{align*}
	Therefore we can bound \begin{align*}
	&\int \norm{\left(\mat{Z}(0)-\mat{Z}(t)\right)\left(\vect{u}(t)-\vect{y}\right) }_F dt\\
	\le &\frac{\poly(n,1/\lambda_0)}{\sqrt{m}} \int \norm{\tilde{\vect{u}}(t)-\vect{y}}_2 dt= \frac{\poly(n,1/\lambda_0)}{\sqrt{m}}.
	\end{align*}
	For the second term, we thus need to bound\begin{align}
	\int_{t=0}^{\infty}\norm{\tilde{\vect{u}}(t)-\vect{u}(t)}_2 dt. \label{eqn:u_tilde_u}
	\end{align}
	To bound Equation~\eqref{eqn:u_tilde_u}, we observe that $\tilde{\vect{u}}(t) \rightarrow \vect{y}$ and $\vect{u}(t) \rightarrow \vect{y}$.
	Therefore, we can choose some $t_0$ such that \begin{align*}
	&\int_{t_0}^\infty\norm{\vect{\tilde{u}}(t)-\vect{u}(t)}_2 dt\\
	\le &\int_{t_0}^\infty(\norm{\vect{\tilde{u}}(t)-\vect{y}}_2  + \norm{\vect{y}-\vect{u}(t)}_2 )dt
	\end{align*}
	Note if we choose $t_0 = \frac{C}{\lambda_0}\left(\frac{m\lambda_0}{n}\right)$ so that \begin{align*}
	\int_{t_0}^\infty\norm{\vect{\tilde{u}}(t)-\vect{u}(t)}_2 dt \le \frac{2\norm{\vect{u}(t)-\vect{y}}_2}{\lambda_0} \le \frac{\poly(n,1/\lambda_0)}{\sqrt{m}}.
	\end{align*}
	Thus it suffices to bound \begin{align*}
	\int_{t=0}^{t_0}\norm{\tilde{\vect{u}}(t)-\vect{u}(t)}_2 dt \le t_0 \max_{0\le t\le t_0} \norm{\tilde{\vect{u}}(t)-\vect{u}(t)}_2.
	\end{align*}
	%First observe that \[
	%\norm{\tilde{\vect{u}}(t)-\vect{u}(t)}_2 \le \int_{\tau = 0}^t \norm{\frac{d\left(\tilde{\vect{u}}(\tau)-\vect{u}(\tau)\right)}{d \tau}}_2 d\tau.
	%\]
	%Note \begin{align*}
	%&\frac{d \left(\tilde{\vect{u}}(t)-\vect{u}(t)\right)}{dt} \\
	%= &-\mat{H}(0)\left(\tilde{\vect{u}}(t)-\vect{y}\right) + \mat{H}(t)\left(\vect{u}(t)-\vect{y}\right) \\
	%= &  -\mat{H}(0)\left(\tilde{\vect{u}}(t)-\vect{u}(t)\right) + \left(\vect{u}(t)-\vect{y}\right)\left(\mat{H}(t)-\mat{H}(0)\right).
	%\end{align*}
	%Since $\mat{H}(0)$ is positive semidefinite, $-\mat{H}(0)\left(\tilde{\vect{u}}(t)-\vect{u}(t)\right) $ term only makes $\norm{\tilde{\vect{u}}(t)-\vect{u}(t)}_2$ smaller.
	%Therefore, we have \begin{align*}
	%&\norm{\tilde{\vect{u}}(t)-\vect{u}(t)}_2 \\
	%\le &\int_{\tau =0}^t \norm{\vect{u}(\tau)-\vect{y}}_2 \norm{\mat{H}(t)-\mat{H}(0)}_2 \\
	%\le & t\norm{\vect{u}(0)-\vect{y}}_2 \frac{\poly(n,1/\lambda_0)}{\sqrt{m}} = \frac{t\poly(n,1/\lambda_0)}{\sqrt{m}} .
	%\end{align*}
	Therefore, we have \begin{align*}
	&\int_{t=0}^{t_0}\norm{\tilde{\vect{u}}(t)-\vect{u}(t)}_2 dt \\
	\le &t_0 \max_{0\le t\le t_0} \norm{\tilde{\vect{u}}(t)-\vect{u}(t)}_2 \\
	\le &t_0^2 \frac{\poly(n,1/\lambda_0)}{\sqrt{m}} \\
	\le &\frac{\poly(n,1/\lambda_0,\log(m))}{\sqrt{m}}.
	\end{align*}
\end{proof}

==> trajectory.tex <==
In this section we present our main characterization of the trajectory.
Our key finding is that both trajectories $\left\{\mat{W}(k)\right\}_{k=0}^\infty$ and $\left\{\vect{u}(k)\right\}_{k=0}^\infty$ can be described by perturbed linear dynamical systems where the perturbation goes to $0$ as the width $m$ goes to infinity.

In the following two subsections, we will give the reference linear dynamical system, then give a perturbation bound that characterize the difference between the actual trajectory generated by the gradient descent algorithm and the reference linear dynamical system.

\subsection{Trajectory of Predictions}
\label{sec:traj_pred}
By some standard calculation, one can find the trajectory of predictions is defined as 
\begin{align*}
	\vect{u}(k+1) = \vect{u}(k) - \eta \mat{H}(k)\left(\vect{u}(k)-\vect{y}\right).
\end{align*}
Now we define our ``unperturbed" linear dynamical system of the trajectory of predictions $\{\tilde{\vect{u}}(k)\}_{k=0}^\infty$
\begin{align}
	\tilde{\vect{u}}(0) = &\vect{u}(0), \nonumber\\
	\tilde{\vect{u}}(k+1) = &\tilde{\vect{u}}(k) - \eta \mat{H}(0)\left(\tilde{\vect{u}}(k)-\vect{y}\right). \label{eqn:u_tilde_dynamics}
\end{align}
Recall $\mat{H}_{ij}(0) = \frac{1}{m}\sum_{r=1}^{m} \indict_{r,i}\indict_{r,j}$ for $(i,j) \in [n] \times [n]$.
%\[\mat{H}^\infty_{ij} = \vect{x}_i^\top \vect{x}_j \expect_{\vect{w}\sim N(\vect{0},\mat{I})}\left[\indict\left\{\vect{w}^\top \vect{x}_i \ge 0, \vect{w}^\top \vect{x}_j \ge 0\right\}\right].\]
This trajectory $\{\tilde{u}(k)\}_{k=1}^{\infty}$ has the same initialization as $\left\{\vect{u}(k)\right\}_{k=0}^\infty$ but at each iteration, $\tilde{\vect{u}}(k)$ uses the initial Gram matrix $\mat{H}(0)$ to do the update and $\vect{u}(k)$ uses Gram matrix $\mat{H}(k)$ which varies at each iteration.
In \cite{du2018provably}, it was shown $\mat{H}(k)$ is close to $\mat{H}^\infty$ if $m$ is large.
Based on this observation, we can show the following perturbation theorem.
\begin{thm}\label{thm:traj_u}
\begin{align}
\norm{\tilde{\vect{u}}(k) - \vect{u}(k)}_2 \le \frac{\poly(n,1/\lambda_0)}{\sqrt{m}}, \forall k \ge 0. \label{eqn:traj_u_perturb}
\end{align}
\end{thm}
This theorem shows, to study the dynamics of $\vect{u}(k)$, we can instead study $\tilde{\vect{u}}(k)$.
Since $\tilde{\vect{u}}(k)$ is a \emph{linear} dynamical system, all information is contained in $\mat{H}(0)$ and initialization $\vect{u}(0)$, we can characterize $\tilde{\vect{u}}(k)$ in a quantitatively precise manner.
We will use this trajectory to explain why true labels converge faster than random labels in Section~\ref{sec:rate}. 






\subsection{Trajectory of Parameters}
\label{sec:traj_W}
Now we consider the dynamics of parameters.
We define the ``unperturbed" linear dynamical system as \begin{align*}
	\widetilde{\mat{W}}(k+1) &= \widetilde{\mat{W}}(k) - \eta\mat{Z}(0)\left(\tilde{\vect{u}}(k)-\vect{y}\right),\\ \widetilde{\mat{W}}(0) &= \mat{W}(0). 
\end{align*}
Recall $\mat{Z}(0)$ is the initial \emph{extended feature matrix}.
Similar to the trajectory of predictions, the following theorem shows $\widetilde{\mat{W}}(k)$ is close to $\mat{W}(k)$ for all$k = 0,1,\ldots,$. 
\begin{thm}\label{thm:traj_W}
For $k=0,1,\ldots$, we have \begin{align}
	\norm{\mat{W}(k)-\widetilde{\mat{W}}(k)}_F \le \frac{\poly(n,1/\lambda_0,\log(m))}{\sqrt{m}} \label{eqn:traj_W_perturb}
\end{align}
\end{thm}

This theorem establishes that if the width is sufficiently large, the linear dynamical system $\{\widehat{\mat{W}}(k)\}_{k=0}^\infty$ identifies the main characteristics of the parameter trajectory $\{\mat{W}(k)\}_{k=0}^\infty$ and therefore we can use this liner dynamical system to analyze the properties of the learned neural network.
In Section~\ref{sec:generalization}, we will exploit this idea to derive a generalization bound.










